A Class of Multiparameter Signless Stirling Numbers of the First Kind and their $q$-Analogues

In this work, we provide a probabilistic derivation of a class of multiparameter signless Stirling numbers of the first kind and their q-analogues, and study the associated multivariate discrete distributions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{158}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2026\\
EPTCS 445, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.445.19}{10.4204/EPTCS.445.19}}
\pdfoutput=1

